Impact Analysis of Baseband Quantizer on Coding Efficiency for HDR Video

Digitally acquired high dynamic range (HDR) video baseband signal can take 10 to 12 bits per color channel. It is economically important to be able to reuse the legacy 8 or 10-bit video codecs to efficiently compress the HDR video. Linear or nonlinear mapping on the intensity can be applied to the baseband signal to reduce the dynamic range before the signal is sent to the codec, and we refer to this range reduction step as a baseband quantization. We show analytically and verify using test sequences that the use of the baseband quantizer lowers the coding efficiency. Experiments show that as the baseband quantizer is strengthened by 1.6 bits, the drop of PSNR at a high bitrate is up to 1.60dB. Our result suggests that in order to achieve high coding efficiency, information reduction of videos in terms of quantization error should be introduced in the video codec instead of on the baseband signal.

==> table_exp.tex <==
    
    \footnotesize
		\begin{tabular}{ccccc}
		  \hline \hline
			\multirow{3}{*}{sequence} 
			& \multicolumn{2}{c}{intra-coding} & \multicolumn{2}{c}{inter-coding} \\ \cline{2-5}
			& \multicolumn{4}{c}{PSNR gap (dB) at extreme BRs} \\ \cline{2-5}
			& low & high & low & high \\ \hline
			BalloonFe. & $0.13$ & $0.83$ & $0.19$ & $0.83$\\ \hline
			Market     & $0.04$ & $0.23$ & $0.03$ & $0.35$ \\ \hline
			Typewriter & $0.29$ & $1.12$ & $0.62$ & $1.60$ \\ \hline
			\hline
		\end{tabular}
		
		
		

==> table_simu.tex <==
    
    \footnotesize
		\begin{tabular}{cccc}
		  \hline \hline
			\multirow{2}{*}{$q_1/q_2$} & \multicolumn{2}{c}{simulation} & \multirow{2}{*}{theory [Eqn.~(\ref{eq:snr_loss})]} \\ \cline{2-3}
			& case (a) & case (b) & \\ \hline
			$1/8$ & $-0.13$ & $-0.16$ & $-0.13$ \\ \hline
			$1/4$ & $-0.51$ & $-0.53$ & $-0.51$ \\ \hline
			$1/2$ & $-1.74$ & $-1.75$ & $-1.76$ \\ \hline
			$1/1$ & $-3.00$ & $-2.95$ & $-2.98$ \\ \hline
			\hline
		\end{tabular}
		

